Efficiently Learning Single-Arm Fling Motions to Smooth Garments

Recent work has shown that 2-arm "fling" motions can be effective for garment smoothing. We consider single-arm fling motions. Unlike 2-arm fling motions, which require little robot trajectory parameter tuning, single-arm fling motions are very sensitive to trajectory parameters. We consider a single 6-DOF robot arm that learns fling trajectories to achieve high garment coverage. Given a garment grasp point, the robot explores different parameterized fling trajectories in physical experiments. To improve learning efficiency, we propose a coarse-to-fine learning method that first uses a multi-armed bandit (MAB) framework to efficiently find a candidate fling action, which it then refines via a continuous optimization method. Further, we propose novel training and execution-time stopping criteria based on fling outcome uncertainty; the training-time stopping criterion increases data efficiency while the execution-time stopping criteria leverage repeated fling actions to increase performance. Compared to baselines, the proposed method significantly accelerates learning. Moreover, with prior experience on similar garments collected through self-supervision, the MAB learning time for a new garment is reduced by up to 87%. We evaluate on 36 real garments: towels, T-shirts, long-sleeve shirts, dresses, sweat pants, and jeans. Results suggest that using prior experience, a robot requires under 30 minutes to learn a fling action for a novel garment that achieves 60-94% coverage.

==> fig_tex/garments.tex <==

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/result_illustration_v02.png}
    \caption{Examples of fling results and corresponding coverage values. Top: Robot fling results during execution time using the best learned action. Bottom: Human smoothed state of each garment, which we mark as ``100\%'' to indicate an upper bound on performance. These garments are in $G_{\rm test}$, with one per category, showing (from left to right) a towel, a T-shirt, and a long-sleeve shirt.}
    \label{fig:result_illustration}
\end{figure}

==> tables/rot_res.tex <==
\subsection{Vertical Rotation Validation}
\label{sssec:Rotation}

As described in Section~\ref{sec:direction-rotation}, we use a convolutional neural network to select the garment's fling direction (i.e., rotation).  We automatically collect 12 training data points given 1 human label. We collect data with 3 T-shirts and 2 towels, each with about 20 different initial configurations, resulting in a dataset of 1,436 total images. We divide these 1,436 images to use 1,148 images for training, 144 for validation and 144 for testing. The CNN classifier is trained with a standard cross entropy loss for 100 epochs, which is when the validation loss roughly converged.
The average absolute error between the predicted rotation angle and the test set label is $15\degree$.

To analyze the benefit of adjusting the initial rotation, we execute the best action found by MAB with 16 actions with CEM refinement on the 3 test garments in $G_{\rm test}$ with and without rotations. For each garment, we randomly rotate the gripper to simulate a random state into which the garment can fall when the gripper grasps the garment in an arbitrary orientation. We then apply the rotation network to observe the garment's vertical orientation and produce a desired rotation correction. We compare the resulting coverage of the same fling action with and without this rotation. The results are shown in Table~\ref{tab:rotation_ablation}. We can see that without rotation, the performance of the fling significantly decreases. While the T-shirt and the long-sleeve shirt achieve similar results with the rotation module compared to the default rotation considered previously, the towel's performance is not as competitive as before, even though it still outperforms the randomized rotation trials without the rotation module. We believe that this is due to the towel's greater sensitivity to the starting configuration and orientation compared to other garments.

\begin{table}[t]
%   \setlength\tabcolsep{5.0pt}
%   \begin{adjustbox}{width=\columnwidth,center}
  \centering
    \begin{tabular}{c|c|c}
    \toprule
                     Garment & Coverage, no rotation & Coverage, with rotation \\ \midrule
    Towel             & 56 $\pm$ 11 \%                     & 76 $\pm$ 20 \%                    \\
    T-shirt           & 62 $\pm$ 12 \%                    & 71 $\pm$ 11 \%                    \\
    Long-sleeve Shirt & 60 $\pm$ \text{ }7 \%                   & 65 $\pm$ \text{ }4 \%                    \\ \bottomrule
    \end{tabular}
%   \end{adjustbox}
  \caption{
  Coverage achieved for the three test garments (plus or minus one standard deviation) by the same learned fling action in 20 test trials starting from a random gripper rotation angle with and without active rotation correction. The results indicate that rotations significantly improve the fling action's effectiveness.
  }
  \vspace*{-0pt}
  \label{tab:rotation_ablation}
\end{table} 
